Porosities and dimensions of measures

We introduce a concept of porosity for measures and study relations between dimensions and porosities for two classes of measures: measures on $R^n$ which satisfy the doubling condition and strongly porous measures on $R$.

==> f1.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point        .59      15.20 {\clap{$b$}                                                  }
\point       1.96      15.20 {\clap{$y$}                                                  }
\point       4.02      15.20 {\clap{\eightpoint{$y+2\delta(c-b)$}}                        }
\point       7.11      15.20 {\clap{\eightpoint{$b+{\textstyle{1\over2}}(1-\delta)(c-b)$}}}
\point      12.02      15.20 {\clap{$y'$}                                                 }
\point      14.31      15.20 {\clap{$c$}                                                  }
\point       2.99      16.55 {\clap{$I_1$}}
\point      13.16      16.55 {\clap{$I_2$}}
\point       8.02      16.31 {\clap{\eightpoint{no mass}}}
 }}


==> f2.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point        .45      13.30 {\clap{$a$}                                                  }
\point       7.95      13.30 {\clap{$b$}                                                  }
\point       8.25      13.30 {\clap{$y$}                                                  }
\point       9.75      13.30 {\clap{\eightpoint{$y+2\delta(c-b)$}}                        }
\point      11.05      13.30 {\clap{$y'$}                                                 }
\point      11.25      12.88 {\rlap{\eightpoint{$b+{1\over2} (1-\delta)(c-b)$}}           }
\point      14.95      13.30 {\clap{$c$}                                                  }
\point      10.00      14.29 {\clap{\eightpoint{$B(z,q'(c-y'))$}}}
\point      11.05      14.99 {\clap{\eightpoint{$B(y',c-y')$}}}
 }}


==> f3.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point        .52      15.20 {\clap{$b$}                                                  }
\point       1.59      15.20 {\clap{$y$}                                                  }
\point       4.27      15.20 {\clap{\eightpoint{$y+2\delta(c-b)$}}                        }
\point       7.27      15.20 {\clap{$y'$}                                                 }
\point       7.70      15.20 {\rlap{\eightpoint{$b+{1\over 2}(1-\delta)(c-b)$}}           }
\point      15.52      15.20 {\clap{$c$}                                                  }
\point       2.66      16.79 {\clap{$I_3$}}
\point      13.38      16.79 {\clap{$I_4$}}
\point       7.49      16.47 {\clap{\eightpoint{$B(z,q'(c-y'))$}}}
 }}


==> f4.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point        .59      15.20 {\clap{$b$}                                                  }
\point       1.74      15.20 {\clap{$y$}                                                  }
\point       6.31      15.20 {\clap{$y'$}                                                 }
\point       4.59      15.20 {\clap{\eightpoint{$y+2\delta(c-b)$}}                        }
\point       7.22      15.20 {\rlap{\eightpoint{$b+{1\over 2}(1-\delta)(c-b)$}}           }
\point      15.45      15.20 {\clap{$c$}                                                  }
\point      10.99      16.79 {\clap{$B(z,q'(c-y'))$}}
\point       5.45      16.31 {\clap{\eightpoint{no mass}}}
 }}


==> fig.tex <==
 \def\point#1 #2 #3 {\rlap{\kern #1 truecm
 \raise #2 truecm \hbox{#3}}}
 \def\spot{{\kern
 -0.2em\lower.55ex\hbox{$\bullet$}}}
 \def\clap#1{{\setbox0=\hbox{#1}\dimen0
 =\wd0\divide\dimen0
 by 2\hskip-\dimen0\box0}}
 \smash{\hbox{
\point       2.88      16.80 {\clap{$D_i^\L$}}
\point       7.45      16.80 {\clap{$D_i$}}
\point      12.02      16.80 {\clap{$D_i^\R$}}
\point       4.59      16.32 {\clap{\eightpoint{$D_i^{\L}(\R)$}}}
\point      10.31      16.32 {\clap{\eightpoint{$D_i^{\R}(\L)$}}}
\point       5.16      14.96 {\clap{\eightpoint{$a_i$}}}
\point       6.31      14.96 {\clap{\eightpoint{$b_i$}}}
\point       7.45      14.96 {\clap{\eightpoint{$c_i$}}}
\point       8.59      14.96 {\clap{\eightpoint{$d_i$}}}
\point       9.74      14.96 {\clap{\eightpoint{$e_i$}}}
\point       1.16      14.24 {\clap{\eightpoint{$p_i^3$}}}
\point       2.31      14.24 {\clap{\eightpoint{$p_i^2$}}}
\point       3.45      14.24 {\clap{\eightpoint{$p_i^2$}}}
\point       4.59      14.24 {\clap{\eightpoint{$p_i$}}}
\point       5.74      14.24 {\clap{\eightpoint{$p_i^2$}}}
\point       6.88      14.24 {\clap{\eightpoint{$p_i$}}}
\point       8.02      14.24 {\clap{\eightpoint{$p_i$}}}
\point       9.16      14.24 {\clap{\eightpoint{$1$}}}
\point      10.31      14.24 {\clap{\eightpoint{$p_i^2$}}}
\point      11.45      14.24 {\clap{\eightpoint{$p_i$}}}
\point      12.59      14.24 {\clap{\eightpoint{$p_i$}}}
\point      13.74      14.24 {\clap{\eightpoint{$1$}}}
 }}


==> xdefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% mechanism for forward referencing %%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This checks whether the defs.lst file contains
%% at least the line
%% \def\nonemeptydefs{}
%% which was written by xdefs
%% Otherwise, we assume 
%% that defs.lst must be completely recreated.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@checkfirstline{\ifundefined{nonemptydefs}
\gdef\@haddefs{F}
\immediate\write16{--------Recreating defs.lst}
\else
\gdef\@haddefs{T}
\immediate\write16{--------Using old defs.lst}
\fi
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% define a new symbol%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@definereally#1#2#3{\expandafter\xdef\csname #1#2\endcsname{#3}\relax}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  write defined symbol to file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@writetofile#1#2#3{%
\write\@defs{\string\expandafter\string\xdef\string\csname}\relax%%
\write\@defs{\string #1#2\string\endcsname{\csname #1#2\endcsname}}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% check whether defs.lst exists%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@haddefs{T}
\gdef\@neednewrun{T}
\gdef\@erasedefs{F}
\gdef\@doubly{F}
\newread\@defs
\openin\@defs defs.lst
\ifeof\@defs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% it does not exist%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\@haddefs{F}
\immediate\write16{*********Creating defs.lst}
\else
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% it exists and now we check if its ``empty''%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\closein\@defs
\input defs.lst
\@checkfirstline
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% now we open it for writing again%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\openout\@defs=defs.lst%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% ... and we write the identification line%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\write\@defs{\string\def\string\nonemptydefs{}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @phaseone creates definitions when defs.lst is recreated from scratch%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@phaseone(#1,#2,#3){\ifundefined{#1#2}%%
\@definereally{#1}{#2}{#3}%%
\@writetofile{#1}{#2}{#3}%%%
\else%%
 \write16{!!!!!doubly defined #1,#2}%%
 \gdef\@doubly{T}%%
\fi%%
}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @phasetwo creates definitions when defs.lst existed.%%
%% it also checks if the definition of the value of a symbol%%
%% has changed (e.g. if the euqtion was moved inside the paper)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@phasetwo(#1,#2,#3){\@undefineda{#1#2}%%
\else%%
\edef\@firstarg{\csname #1#2\endcsname}%%
\edef\@secondarg{#3}%%
\ifnum \@stringcompare{\@firstarg}{\@secondarg} = 0%%
\else%%
\immediate\write16{ definition of #1 #2 changed : \@firstarg  --->\@secondarg}%%
\gdef\@neednewrun{T}%%
\gdef\@erasedefs{T}%%
\fi%%
\fi%%
\@definereally{#1}{#2}{#3}%%
\@writetofile{#1}{#2}{#3}}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% check if symbol was never defined (used when defs.lst already exists)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@undefineda#1{\expandafter\ifx\csname#1\endcsname\relax%%%
{\gdef\@neednewrun{T}%%
 \immediate\write16{*********** used #1 which was never defined }}}%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% redefinition of NEWDEF depending on whether defs existed%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if F\@haddefs%%
 \def\NEWDEF #1,#2,#3 {\@phaseone({#1},{#2},{#3})}%%
\else%%
 \def\@neednewrun{F}%%
 \let\ifundefined=\@undefineda%%
 \def\NEWDEF #1,#2,#3 {\@phasetwo({#1},{#2},{#3})}%%
\fi%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% messages when \bye is encountered (you cannot use \end)%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bye{\if T\@erasedefs%%
 \write16{**** I suspect doubly defined tokens ****}%%
 \write16{**** I erase defs.lst now ***********}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% next line ``erases'' defs.lst so that it will be%%
%% recreated in the next run%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \openout\@defs=defs.lst%%
\fi%%
\if T\@doubly%%
 \write16{**** There are doubly defined tokens *****}%%
 \write16{**** You have to correct the TeX file and rerun *****}%%
\fi%%
\if T\@neednewrun%%
 \write16{*********NEED ANOTHER RUN************}%%
\fi%%
\end}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@stringcompare#1#2{\expandafter\@strcompa#1|===#2|===}%%
\def\@strcompa#1===#2==={\expandafter\@strcompb#2===#1===}%%
\def\@strcompb#1===#2==={\@compcont#1\\#2\\}%%
\def\@compcont#1#2\\#3#4\\{%%%
\csname @comp%%%
 \if #1#3\if #1|same\else contt\fi%%
   \else diff\fi%%
  \endcsname #2\\#4\\}%%
\def\@compcontt#1#2\\#3#4\\{\@strcompb#1#2===#3#4===}%%
\def\@compsame#1\\#2\\{0}%%
\def\@compdiff#1\\#2\\{1}%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=\active
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% EOF xdefs.tex %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
